A Joint Network for Grasp Detection Conditioned on Natural Language Commands

We consider the task of grasping a target object based on a natural language command query. Previous work primarily focused on localizing the object given the query, which requires a separate grasp detection module to grasp it. The cascaded application of two pipelines incurs errors in overlapping multi-object cases due to ambiguity in the individual outputs. This work proposes a model named Command Grasping Network(CGNet) to directly output command satisficing grasps from RGB image and textual command inputs. A dataset with ground truth (image, command, grasps) tuple is generated based on the VMRD dataset to train the proposed network. Experimental results on the generated test set show that CGNet outperforms a cascaded object-retrieval and grasp detection baseline by a large margin. Three physical experiments demonstrate the functionality and performance of CGNet.

==> res3D.tex <==
\subsection{3D dense reconstruction}


==> resBaselines.tex <==
\subsection{Vision}

==> resFit.tex <==
\subsection{Primitive shapes fitting}

==> resGrasping.tex <==
\subsection{Grasping experiments}


==> resMultiview.tex <==
\subsection{Multi-view object pose fusion}


==> resPhyFig.tex <==
\begin{figure}[t!]
  \centering
  \begin{tikzpicture}[inner sep = 0pt, outer sep = 0pt]
    \node[anchor=south west] at (0in,0in)
      {{\includegraphics[width=1\columnwidth,clip=true,trim=0in 0in 0in 0in]{figures/results_phy.pdf}}};
%   \node[anchor=north west,xshift=380pt,yshift=-15pt] at (SF.north west) {(b)};
%    \node[yshift=-2pt,anchor=south] at (0.3\columnwidth,0.1in) {\bf \small (a)};
%    \node[yshift=-2pt,anchor=south] at (0.75\columnwidth,0.1in) {\bf \small (b)};
%    \node[yshift=-2pt,anchor=south] at (4.70in,0.5in) {\bf \small (c)};
%    \node at (2.6in,1.2in) {$\primSeg_{i_1}$};
%    \node at (2.6in,0.8in) {$\primSeg_{i_2}$};
%    \node at (3.75in,1.2in) {$\primShape_{j_1}$};
%    \node at (3.75in,0.8in) {$\primShape_{j_2}$};
    \node at (0.3\columnwidth,-0.05in) {\textbf{(a)}};
    \node at (0.75\columnwidth,-0.05in) {\textbf{(b)}};
  \end{tikzpicture}%
  \caption{Grasp detection results in physical experiments
    \textbf{(a)} Physical experiment settings.
 Manipulator is a 7-DOF robotic arm;
    \textbf{(b)} Example detection results for overlapping multi-objects physical experiment.%
    \label{fig:resPhy}}
\end{figure}


==> resSeg.tex <==
\subsection{Primitive shapes segmentation}

